Faster Algorithms for Global Minimum Vertex-Cut in Directed Graphs

We study the directed global minimum vertex-cut problem: given a directed vertex-weighted graph $G$, compute a vertex-cut $(L,S,R)$ in $G$ of minimum value, which is defined to be the total weight of all vertices in $S$. The problem, together with its edge-based variant, is one of the most basic in graph theory and algorithms, and has been studied extensively. The fastest currently known algorithm for directed global minimum vertex-cut (Henzinger, Rao and Gabow, FOCS 1996 and J. Algorithms 2000) has running time $\tilde{O}(mn)$, where $m$ and $n$ denote the number of edges and vertices in the input graph, respectively. A long line of work over the past decades led to faster algorithms for other main versions of the problem, including the undirected edge-based setting (Karger, STOC 1996 and J. ACM 2000), directed edge-based setting (Cen et al., FOCS 2021), and undirected vertex-based setting (Chuzhoy and Trabelsi, STOC 2025). However, for the vertex-based version in directed graphs, the 29 year-old $\tilde{O}(mn)$-time algorithm of Henzinger, Rao and Gabow remains the state of the art to this day, in all edge-density regimes. In this paper we break the $\Theta(mn)$ running time barrier for the first time, by providing a randomized algorithm for directed global minimum vertex-cut, with running time $O\left(mn^{0.976}\cdot\operatorname{polylog} W\right)$ where $W$ is the ratio of largest to smallest vertex weight. Additionally, we provide a randomized $O\left(\min\left\{m^{1+o(1)}\cdot k,n^{2+o(1)}\right\}\right)$-time algorithm for the unweighted version of directed global minimum vertex-cut, where $k$ is the value of the optimal solution. The best previous algorithm for the problem achieved running time $\tilde O\left(\min\left\{k^2 \cdot m, mn^{11/12+o(1)}, n^{2+o(1)}\right\}\right)$ (Forster et al., SODA 2020, Li et al., STOC 2021).

==> graph-modification-steps.tex <==
\subsection{Graph Modification Steps}
\label{subsec: graph modification}
\mynote{is this used? If not should be deleted}
Suppose we are given a directed graph $G$ with integral weights $w(v)\geq 1$ on its vertices $v\in V(G)$. Assume further that we are given two vertices $s,t\in V(G)$, such that there is no edge connecting $s$ to $t$ in $G$. Let $(L,S,R)$ be an arbitrary fixed global minimum vertex-cut, that we refer to as the \emph{distinguished min-cut}.
One of the methods that our algorithm uses is to gradually sparsify the graph $G$, while preserving the value of the minimum $s$-$t$ vertex-cut, provided that $s\in L$ and $t\in R$ holds, where $(L,S,R)$ is the distinguished min-cut. 
We now define graph modification steps that our algorithm may perform, which are of the following three types.

\paragraph{Type-1 graph modification step:} given an aribtrary vertex $v\in V(G)\setminus\set{s,t}$, add an edge $(v,t)$ to $G$. If $s\in L$ and $t\in R$ (where $(L,S,R)$ is the distinguished global minimum vertex-cut), then this modification step is \emph{valid} iff $v\in S\cup R$. If $s\not\in L$ or $t\not\in R$, then the modification step is always valid.

\paragraph{Type-2 graph modification step:} given an arbitrary vertex $v\in V(G)\setminus\set{s,t}$, such that the edge $(v,t)$ currently lies in $G$, and an edge $e=(v,u)\in \delta^+(v)\setminus\set{(v,t)}$, delete $e$ from $G$. This modification step is always valid.


%\paragraph{Type-3 graph modification step:} given a vertex $v\in V(G)\setminus\set{s,t}$, increase $w(v)$ to $\wmax$.  If $s\in L$ and $t\in R$ (where $(L,S,R)$ is the distinguished global minimum vertex-cut), then this modification step is valid iff $v\in L$. If $s\not\in L$ or $t\not\in R$, then the modification step is always valid.\mynote{\textcolor{blue}{I think we may not be using type-3 graph modification steps anywhere in the paper. - Ron}}

\paragraph{Type-3 graph modification step:} given an edge $e=(u,v)\in E(G)$, delete $e$ from $G$. This step is valid if $(s,v)\in E(G)$ and $u\neq s$. % there exists a path $P$ connecting $s$ to $v$ in $G$, such that the weight of every inner vertex of $P$ is $\wmax$ and $e\not\in E(P)$ (note that it is possible that $P$ consists of a single edge $(s,v)$).

The following observation summarizes the properties of graph modification steps.

\begin{observation}\label{obs: graph modification} Let $G$ be a directed graph with integral weights $w(v)\geq 1$ on its vertices $v\in V(G)$ and let $s,t\in V(G)$ be two vertices for which $(s,t)\not\in E(G)$. Let $(L,S,R)$ be an arbitrary global minimum vertex-cut in $G$ that we refer to as the distinguished cut, and let $C$ denote the value of the minimum $s$-$t$ vertex-cut in $G$. Finally, $\hat G$ be the graph obtained from $G$ after executing a sequence of valid graph modification steps (with respect to the cut $(L,S,R)$), and let $C'$ be the value of  the minimum $s$-$t$ vertex-cut in $\hat G$. Then $C'\geq C$ holds. Moreover, if  $s\in L$ and $t\in R$ hold, then $C'=C$.
\end{observation}

\begin{proof}
We start by proving that a sequence of valid modification steps cannot decrease the value of the minimum $s$-$t$ vertex cut, using the following observation.

\begin{observation}\label{cl : graph modification steps do not reduce vertex cut below wmax}
	Let $\tilde G$ be the graph that is obtained from $G$ after performing a sequence of valid graph modification steps, and let $\tilde C$ denote the value of the minimum $s$-$t$ vertex cut in it. Let $\tilde G'$ be obtained from $\tilde G$ by performing one additional valid graph modification step, and let $\tilde C'$ be the value of the minimum $s$-$t$ vertex cut in $\tilde G'$. Then $\tilde C'\geq \tilde C$.
\end{observation}


\begin{proof}
Consider the graph $\tilde G$ that is obtained from $G$ via a sequence of valid modification steps, and let $\tilde G'$ be obtained from $\tilde G$ by performing one additional valid modification step. Recall that we denoted the values of the minimum $s$-$t$ vertex-cut in $\tilde G$ and $\tilde G'$ by $\tilde C$ and $\tilde C'$, respectively, and our goal is to prove that $\tilde C'\geq \tilde C$. 
Consider now the modification step that was applied to $\tilde G$ to obtain $\tilde G'$. We distinguish between $3$ cases, depending on the type of the modification step.

\paragraph{Type-1 modification step:} Type-1 modification step inserts an edge into $\hat G$. This modification clearly cannot decrease the value of the minimum $s$-$t$ cut, so $\tilde C'\geq \tilde C$ holds.

\paragraph{Type-2 modification step:}
Recall that in a type-2 modification step, we delete an edge $(v,u)$ from the graph, where $v$ is a vertex of $V(\tilde G)\setminus\set{s,t}$ with an edge $(v,t)\in E(\tilde G)$, and $u\neq t$.
Consider the maximum vertex-capacitated $s$-$t$ flow $f$ in $\tilde G$, and recall that its value, from the Max-Flow / Min-Cut theorem is equal to $\tilde C$. Let $\pset$ be a flow-path decomposition of $f$. If no path in $\pset$ contains the edge $e$, then $f$ remains a valid $s$-$t$ flow in $\tilde G'$. Otherwise, let $P\in \pset$ be a flow-path that contains $e$, and let $P'\subseteq P$ be its subpath from $s$ to $v$. We then replace $P$ with the path $P'\circ(v,t)$ that lies in $\tilde G'$, obtaining a valid $s$-$t$ flow in $\tilde G$, whose value remains equal to $\tilde C$. We perform this transformation to every path of $\pset$ that contains $e$. It is immediate to verify that the new flow is contained in $\tilde G'$, has value $\tilde C$, and does not violate the capacities of the vertices. From the Max-Flow / Min-Cut theorem, we then get that $\tilde C'\ge \tilde C$.

%\paragraph{Type-3 modification step:} in a type-3 modification step we increase the weight of some vertex $v\in V(G)\setminus\set{s,t}$. It is immediate to verify that this modification cannot decrease the value of the minimum $s$-$t$ vertex-cut and so $\tilde C'\ge \tilde C$ must hold.

\paragraph{Type-3 modification step:}
Recall that in a type-3 modification step, we delete an edge $e=(u,v)$ from the graph, and the step is valid iff edge $(s,v)$ currently lies in the graph $\tilde G$  and $u\neq s$.

Consider the maximum vertex-capacitated $s$-$t$ flow $f$ in $\tilde G$, and recall that, from the Max-Flow / Min-Cut theorem its value is $\tilde C$.
Let $\pset$ be the flow-path decomposition of $f$. 
 We will modify the flow $f$ to obtain a valid flow $f'$ in $\tilde G'$ of the same value. From the Max-Flow / Min-Cut theorem, it will then follow that $\tilde C'\geq \tilde C$.

In order to modify the flow $f$, we consider its flow-path decomposition $\pset$. Let $\pset'\subseteq \pset$ be the collection of all paths that contain the vertex $v$, and let $\pset''=\pset\setminus\pset'$. For every path $Q\in \pset'$, let $Q'\subseteq Q$ be the subpath of $Q$ from $v$ to $t$, and let $\hat Q=(s,v)\circ Q'$. Observe that $\hat Q$ is a valid $s$-$t$ path in graph $\tilde G'$. Consider now the flow $f'$ in $\tilde G'$, where, for every path $Q\in \pset''$, we send $f(Q)$ flow units via $Q$, and for every path $Q\in \pset'$, we sent $f(Q)$ flow units via $\hat Q$. It is easy to see that the resulting flow obeys all vertex capacities in $\tilde G'$. Moreover, the value of the flow is $\val(f')=\val(f)=\tilde C$. Therefore, $\tilde C'\geq \tilde C$.
\end{proof}

We are now ready to complete the proof of \Cref{obs: graph modification}. From \Cref{cl : graph modification steps do not reduce vertex cut below wmax}, $C'\geq C$ must hold. We now prove that, if $s \in L$ and $t \in R$, then $C=C'$ holds.
Since we have already shown that $C' \geq C$, it only remains to show that $C' \leq C$ in this case.
Observe that, if $s \in L$ and $t \in R$, then no valid graph modification step may add an edge connecting a vertex of $L$ to a vertex of $R$. Indeed, in a type-1 modification step, an edge $(v,t)$ is inserted into $G$ but $v\not\in L$ must hold, and in type-2 and type-3 modification steps we only delete edges. 
It is then immediate to verify that, after a sequence of valid graph modification steps, $(L,S,R)$ remains a valid vertex-cut in the resulting graph $\hat G$ of value $C$. We conclude that $C'=C$ in this case. 
\end{proof}


